Discourse-Aware Soft Prompting for Text Generation

Current efficient fine-tuning methods (e.g., adapters, prefix-tuning, etc.) have optimized conditional text generation via training a small set of extra parameters of the neural language model, while freezing the rest for efficiency. While showing strong performance on some generation tasks, they don't generalize across all generation tasks. We show that soft-prompt based conditional text generation can be improved with simple and efficient methods that simulate modeling the discourse structure of human written text. We investigate two design choices: First, we apply \textit{hierarchical blocking} on the prefix parameters to simulate a higher-level discourse structure of human written text. Second, we apply \textit{attention sparsity} on the prefix parameters at different layers of the network and learn sparse transformations on the softmax-function. We show that structured design of prefix parameters yields more coherent, faithful and relevant generations than the baseline prefix-tuning on all generation tasks.

==> figs/plot.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel=$x$,
        ylabel=$y$,
        xmin=0, xmax=30,
        ymin=0, ymax=100,
        xtick={10,20,30},
        ytick={10,20,30,40,50,60,70,80,90,100}
        ]
    \addplot[smooth,mark=*,blue] plot coordinates {
        (0,10)
        (8,30)
        (16,40)
    };
    \addlegendentry{Case 1}

    \addplot[smooth,color=red,mark=x]
        plot coordinates {
            (4,15)
            (10,25)
            (15,40)
            (18,60)
        };
    \addlegendentry{Case 2}
    \end{axis}
    \end{tikzpicture}
    
% \begin{figure}
%   \centering
%   \begin{subfigure}[b]{0.45\textwidth}
% %%%    \begin{adjustbox}{width=\linewidth} % rescale box
%     \begin{tikzpicture}
%       \begin{axis}[
% %%%        width=\linewidth,            % or modify the plot width
%         axis y line = middle,
%         ...
%         ...
%       \end{axis}
%     \end{tikzpicture}
% %%%  \end{adjustbox}       %
% \end{subfigure}%
%   \hfill
%   \begin{subfigure}[b]{0.45\textwidth}
  
  
%  \begin{figure}
%  \centering
% \subimport{figs/}{plot.tex}
\pgfplotsset{footnotesize,samples=10}
\begin{center}% note that \centering uses less vspace...
\begin{tikzpicture}
\begin{axis}[
legend columns=-1,
legend entries={$(x+0)^k$;,$(x+1)^k$;,$(x+2)^k$;,$(x+3)^k$},
legend to name=named,
title={$k=1$}]
\addplot {x};
\addplot {x+1};
\addplot {x+2};
\addplot {x+3};
\end{axis}
\end{tikzpicture}
%
\begin{tikzpicture}
\begin{axis}[title={$k=2$}]
\addplot {x^2};
\addplot {(x+1)^2};
\addplot {(x+2)^2};
\addplot {(x+3)^2};
\end{axis}
\end{tikzpicture}
%
\begin{tikzpicture}
\begin{axis}[title={$k=3$}]
\addplot {x^3};
\addplot {(x+1)^3};
\addplot {(x+2)^3};
\addplot {(x+3)^3};
\end{axis}
\end{tikzpicture}
\\
\ref{named}
\end{center}

==> old/conclusion.tex <==
% ###############
\section{Conclusion and Limitations}
% ###############
We have described simple but effective prompt design options for prefix-tuning of text generation tasks. We enrich prefix parameters with structural biases by way of: prefix-blocking at different layers of the network, sparsity on prefix-parameters and an ensemble of both biases. We show with quantitative and human evaluations on metrics such as coherence and faithfullness that discourse aware prefix designs outperforms baseline prefix-tuning across all text generation tasks even at low data settings and perform at par with finetuning. 


We note a few limitations of our work: (1) our experiments are limited by available datasets, and only evaluated on limited closed domain text generation tasks; (2) we focused on efficient prefix-tuning, while ensemble of different efficient tuning models can boost performance even further; (3) we conduct experiments with ${\small \sim}$300M parameter models as in past work, but it will be valuable for future work to scale to larger models which may exhibit more coherent generations. 


% Future work might focus on prefix-tune architectures for imbuing prefixes with context related knowledge for text generation, combining other efficient tuning methods for performance boost and investigations on other transformer architectures to improve the state-of-the-art. 

% ###############
\section{Ethics Statement}
% ###############
\label{ethics}
In this work we apply several changes to the state-of-the-art encoder-decoder modeling architecture and build several models to benchmark our new architecture with baseline architectures on several open source text generation datasets. 

\paragraph{Intended use.}
Our architecture is designed to build models of abstractive document summarization and table summarization. Potentially our architecture could be used to train models for summarizing any type of datasets (e.g., any documents, textual conversational dialogues, blog posts, reports, meetings, legal forms, etc.) to further improve the productivity and efficiency of the users in their daily activities without needing to read/listen to long documents/conversations/meetings.  


\paragraph{Failure mode.}
Even though our models yield factually consistent summaries, as judged by us and raters, they can still generate factually inconsistent summaries or sometimes hallucinate information that the source document does not include. This might be due to the bias or noise in the training data. Model builders wanting to use our architecture to build models on their datasets should build models with consideration of intellectual properties and privacy rights. 


\paragraph{Misuse Potential.} We note the models to be built with our architecture should be used with careful consideration especially if used to build summarization models. The generated summaries produced by our models are not controlled and use generative approaches, therefore, they could generate unreliable text. Researchers working on abstractive summarization should focus on generating factually correct, ethical and reliable text. If our models are trained on news datasets, a careful consideration should be made on factuality of the generated text and measures have been taken to prevent model hallucinations.  


==> old/experiments.tex <==

\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l l c}
        \hline 
        Dataset & Domain & \#Data  \\
         \hline
         \textbf{Summarization} & & Train/Val/Test \\
         \hline
         XSum (\citeyear{narayan-etal-2018-dont}) &  News &  204K/11K/11K  \\
         CNN/DM (\citeyear{hermann2015teaching})   &  News &  287K/13K/11K \\
         Wikihow (\citeyear{koupaee2018wikihow}) & DIY & 157K/5.6K/5.6k   \\
         SAMSum (\citeyear{gliwa2019samsum})   &  Dialog &   15.7K/<1K/<1K \\
         Pubmed (\citeyear{cohan-etal-2018-discourse})  & Clinical & 203K/6K/6K   \\
         \hline
         \textbf{Structure to Text (S2T)} & & \\
         \hline
         E2E (\citeyear{novikova2017e2e,e2e})  & Reviews & 33K/4K/4.7K   \\
         DART (\citeyear{nan2021dart}) & Reviews& 63K/7K/12.5K\\
        \hline
    \end{tabular}
    \vspace{-8pt}
    \caption{\small Datasets used in the experiments.}
    \label{tab:datasets}
    \vspace{-0.3cm}
\end{table}

\begin{table*}[t]
    \centering
    \footnotesize
    % \resizebox{1\textwidth}{!}{%
    \begin{tabular}{@{}llllll@{}}
        \hline 
        & \multicolumn{1}{c}{\textbf{XSum}}   &  \multicolumn{1}{c}{\textbf{CNN/DM}}   & \multicolumn{1}{c}{\textbf{PubMed}}  & \multicolumn{1}{c}{\textbf{Wikihow}}  & \multicolumn{1}{c}{\textbf{SAMSum}}\\
        \textbf{Method} & \multicolumn{1}{c}{\textbf{R1/R2/R-L}} &
        \multicolumn{1}{c}{\textbf{R1/R2/R-L}} & \multicolumn{1}{c}{\textbf{R1/R2/R-L}} & \multicolumn{1}{c}{\textbf{R1/R2/R-L}} & \multicolumn{1}{c}{\textbf{R1/R2/R-L}} \\
         \hline
        %  & \textbf{0}/\textbf{0}/\textbf{0} & \textbf{0}/\textbf{0}/\textbf{0} & \textbf{0}/\textbf{0}/\textbf{0} & \textbf{0}/\textbf{0}/\textbf{0} & 0/0/0 & \textbf{} \\
        % GEM-T5L & \textbf{0}/\textbf{0}/\textbf{0} & \textbf{0}/\textbf{0}/\textbf{0} & \textbf{0}/\textbf{0}/\textbf{0} & \textbf{0}/\textbf{0}/\textbf{0} & 0/0/0 & \textbf{} \\
        % \hline
                
         \multicolumn{6}{l}{{\textbf{Fineune (FT)}}} \\
         \hline
          FT \textbf{[*]}    & 
          45.14/22.27/37.25 $\color{blue}{\spadesuit}$ &
          44.16/\textbf{21.28}/40.90 $\color{blue}{\spadesuit}$ &
          \textbf{45.09}/\textbf{19.56}/27.42 $\color{blue}{\blacklozenge}$  & 
          42.86/\textbf{19.71}/34.80 $\color{blue}{\blacklozenge}$  & 
          49.30/25.60/47.70 $\color{blue}{\star}$  \\
          FT (repr.). & 
           \textbf{45.47}/\textbf{22.40}/\textbf{37.42} & 
           \textbf{44.30}/21.14/\textbf{41.22} & 
           44.96/19.00/\textbf{27.74}& 
           \textbf{43.26}/19.38/\textbf{34.89} &
          \textbf{53.02}/\textbf{28.30}/\textbf{48.73}   
          \\
          \hline
         \multicolumn{6}{l}{{\textbf{PrefixTune (PT)}}} \\
         \hline

        PT \textbf{[*]}    & 
         43.80/\textbf{\underline{20.93}}/36.05 $\color{blue}{\clubsuit}$ &
         \multicolumn{1}{c}{-} & 
         \multicolumn{1}{c}{-} &  
         \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
         
        PT (repr.)  & 
        43.43/20.37/35.47 & 
        42.50/19.52/39.08 &  
        42.38/16.31/24.57 & 
        39.26/15.58/28.27 &  
        52.12/26.52/48.05
        \\
        UniBlock & 
         43.49/20.58/35.80 &
         42.43/19.38/39.15 &
         42.81/16.96/25.73 & 
         39.34/15.55/28.75&
         52.42/27.70/48.12
         \\
        HierBlock & \textbf{\underline{43.91}}/20.83/\textbf{\underline{36.38}} &
         \textbf{\underline{43.33}}/\textbf{\underline{20.27}}/\textbf{\underline{40.12}} &
         \textbf{\underline{43.16}}/\textbf{\underline{16.83}}/\textbf{\underline{24.87}} & 
         \textbf{\underline{40.03}}/\textbf{\underline{15.90}}/\textbf{\underline{30.15}}& 
         \textbf{\underline{52.68}}/\textbf{\underline{27.88}}/\textbf{\underline{48.56}}
         \\
        %  UniBlock (ours)  &  42.91/{19.64}/34.61 & 42.04/19.50/29.16 & 38.93/14.24/22.63 & {39.31}/{16.60}/{30.85} & 51.07/26.50/42.53 & 30.82\\
        %  HierBlock (ours) \ \  & {42.99}/19.56/{34.76} & {43.04}/{20.21}/{29.73}  & {39.10}/{14.50}/{22.91} & 39.10/16.42/30.59& {51.53}/{26.83}/{42.94}& {31.66}\\
   \hline
    \end{tabular}
    % }
    \vspace{-0.3cm}
    \caption{\small \textbf{Summarization}: \textbf{Prefix blocking} experiment results comparing against finetuning and prefix-tuning. Top block are best reported BART-LARGE models from corresponding papers, middle block are our replication of finetuned and prefix-tuned BART models. Bottom block are our new prefixtuned models: Uniform (UniBlock) and Hierarchical (HierBlock)  prefix blocking represent models which use prefix-blocking at different layers of the network ($\S$~\ref{prefixblocking}). All models use BART-large as backbone, expect a few previously reported model results \textbf{[*]}: $\color{blue}{\spadesuit}$ \citep{lewis-etal-2020-bart}, $\color{blue}{\clubsuit}$ \citep{prefixtune}, $\color{blue}{\star}$\citep{samsumbartlarge}, $\color{blue}{\blacklozenge}$ \citep{pegasus}. The best finetune result accross models (top block) are \textbf{bolded}, best prefixtune models (bottom block) are further \underlined{\textbf{underlined}}. All hyper-parameters are summarized in Appendix Table~\ref{apptable:hyperparameters}.}
    \label{tab:res1}
\end{table*}


% ################################
\section{Experiment Setup}
\label{setup}
% ################################
\noindent{\textbf{Methods.}} 
All of the models are
based on \textsc{Bart-Large} \citep{lewis-etal-2020-bart}, though our methods can be applied to any architecture.
We compare our discourse aware prefix-tuning approaches to full parameter fine-tuning and baseline prefix-tuning \citep{prefixtune}. Finetuning updates all the LM parameters, while all prefix-tuning models freeze LM parameters and only update the prefix parameters. Baseline prefix-tuning models update prefix parameters at each layer (full-stack) of the transformers using dense attention while our proposed models use variations of sparse and blocked attention at different layers of the network.  
We choose the best models on validation dataset during training and repeat each
experiment $\sim$2-3 times with different random seeds and report the average results. For details of the setup see Appendix~\ref{app:hyperparameters}. 
 

\noindent{\textbf{Datasets.}}
\label{datasetsintext}
We conduct experiments across six datasets on two tasks: abstractive summarization and structure-to-text (S2T) generation. We present a summary of the datasets in Table~\ref{tab:datasets} and provide more details about the datasets in Appendix~\ref{app:dataset_details}.

\noindent{\textbf{Metrics.}} For all the tasks and datasets we use the \textit{n}-gram match metrics: ROUGE-1/2/L \citep{lin-2004-rouge} for summarization and BLEU \citep{bleu}, NIST \citep{nist}, METEOR \citep{meteor}, ROUGE-L, TER, Movers \citep{moverscore} and BERTScore \citep{bertscore} for data-to-text generation tasks. We also report human evaluations to 
compare the results of the models on various qualitative evaluation criteria.

% ################################
\section{Experiment Results}
% ################################

% ################################################
\subsection{Are all prefix-parameters useful?}
\label{exp:prefixanalysis}
% ################################################
\noindent\textbf{Finding:} 
Prefix-tuning models encode diverse but task specific features at each layer differently, while the top-layer prefixes encode abstract features.
% Prefix parameters at the top layers encode high-level concepts related to the downstream generation tasks, while models perform better when prefix-parameters are used at all layers. 

\noindent\textbf{Analysis:} 
Earlier work \citep{jiang-etal-2021-enriching,Elazar2021AmnesicPB,beyondbert} suggests that 
some layers of the transformers are better than others at producing representations that are useful for a given task.
To investigate if similar patterns show up in prefix-tuned models, we take XSum dataset and train models with prefix parameters only at the top layers, the bottom layers, and at a single layer.
\begin{table}[h]%
\centering
\parbox{0.2\textwidth}{
\begin{footnotesize}
    \begin{tabular}{@{}l@{}c@{} }
        \hline 
        \footnotesize Layers \ & Rouge-1/2/L \\
         \hline
         \hline
        Top (8-12) \ \ &  42.3/18.1/34.6  \\
        Low (1-7) &  33.7/13.1/26.9   \\
        \hline
        All (1-12) &  42.6/19.3/34.8   \\
        \hline
    \end{tabular}

\end{footnotesize}
\vspace{-0.3cm}
\caption{\footnotesize Validation Rouge scores of prefix-tuned models on XSum using only top/low layers.}
\label{tab:minirouge}
}
\qquad
\begin{minipage}[c]{0.2\textwidth}%
\centering
    % \includegraphics[width=1\textwidth]{figs/eig_bottomlayers.png}
    \begin{tikzpicture}[yscale=0.32,xscale=0.40]
\begin{axis}[
font=\fontsize{15}{0}\selectfont,
xlabel=Layers,
% ylabel=Error
]
\addplot[color=red,mark=x] coordinates {
(1,	27.8497)
(2,27.9531)
(3,28.5052)
(4,28.5875)
(5,28.5239)
(6,28.7596)
(7,29.0929)
(8,29.38)
(9,33.0148)
(10,33.3243)
(11,33.9351)
(12,34.0272)
};
\end{axis}
\end{tikzpicture}
\vspace{-0.4cm}
\captionof{figure}{\footnotesize Validation \textbf{Rouge-L} on single-layer prefix-tuning with XSum.}
\label{fig:singlelayers}
\end{minipage}
\end{table}

 
% We start investigating the impact of prefix parameters at different parts of the transformer network to understand how much these parameters contribute to the task specific performance. Our motivation originates from the previous work \citep{jiang-etal-2021-enriching,Elazar2021AmnesicPB,beyondbert} that suggests that 
% some layers of the transformer models are better than others at producing representations that are useful for a given task. 
% To investigate if similar patterns show up in prefix-tuned models, we build several prefix-tuning models by varying the prefix features at different layers. Using XSum training dataset, we build models with prefix parameters only at the top layers, bottom layers, and each individual layer. 

% \vspace{-0.3cm}
We show layer-specific prefix-tuned models' validation performance results in Table~\ref{tab:minirouge}. The 'Top' layers model is tuned with only the top-layer prefix parameters (i.e., top 4 layers have additional prefix parameters), the 'Low' layers model uses only the lower-layer prefix-parameters (i.e., bottom 7 layers have additional prefix parameters) and 'All' layers prefix parameters is same as baseline prefix-tuning. On inspection, we see a large performance gap between the models trained with top/lower layers up to 6.4 Rouge-1 scores, while we obtain the best performance when we tune all-layer prefix parameters. We see similar patterns on the SAMSum dialog summarization and E2E structure to text generation tasks (details in Appendix~\ref{app:layerwiseprefix}). We also build models when prefix parameters are used at a single layer of the network.  Our analysis on single layers in Figure~\ref{fig:singlelayers} suggest that the top layer prefixes can encode summary related abstract information. 



% ########################################
\subsection{Are hierarchical prompts effective?} 
\label{blockingresults}
% ########################################
\noindent\textbf{Finding:} Hierarchical design of prefix parameters can yield more robust information transfer in text generation outperforming baseline prefix-tuning.

% Hierarchical design of prefix parameters improves long document abstractive summarization tasks by up to 1-2 points on ROUGE metrics compared to the baseline prefix-tuning. 

\noindent\textbf{Analysis:} 
To simulate learning the discourse related representations we bias prefix parameters with a structure of  input documents (as discussed in $\S$\ref{discourse}) and experiment with two hierarchical structures: \textit{uniform} (UniBlock) and \textit{hierarchical} (HierBlock) from $\S$~\ref{prefixblocking}. 
In Table~\ref{tab:res1} we report the performance of our models in comparison to fine-tuning and baseline prefix-tuning on abstractive summarization tasks.  Our results indicate that prefix-blocking
models improve over the baseline prefix-tuning 
on all summarization tasks by up to +1.0 ROUGE score overall, and trailing fine-tuning as low as +1.0 ROUGE score. Especially for Wikihow, which are considered long document summarization task, we observe up to +2 ROUGE-L score improvement. 
% In addition, the performance gap is larger in news article summarization compared to SAMSum conversational summarization dataset.
% The reason behind this may be that SAMSum input tokens are shorter and hierarchical discourse structure is not prominent as much as in the long document encoding tasks.
We further observe that hierarchical blocking on prefixes also helps for structure-to-text tasks, though the performance impact of structural bias is more prominent in summarization tasks. We show detailed results of structure-to-text tasks and provide samples of generated outputs in Appendix~\ref{app:hierpromptdesign}. 
% We conclude from these results that the prefix models tuned with structurally biased additional set of parameters can yield more robust information transfer outperforming finetuning models.   
% We provide samples of generated outputs in Appendix~\ref{app:hierpromptdesign}. 
% We will analyze the results of hierarchical structural design with sparsity under sparsity in $\S$~\ref{doessparseattentionlhelp}.




% \vspace{-0.5cm}
% ################################################
\subsection{Does sparse attention help prefix-tuning?}
\label{doessparseattentionlhelp}
% ################################################
\noindent\textbf{Finding:} With hierarchically structured sparsity training, prefix tuning show more sparse patterns at the lower layers. Sparse prefix parameters at lower layers, and dense at higher layers enable more efficient tuning of the prefix-parameters.
Details on spectrum analysis are provided in Appendix~\ref{app:spectrum} and Appendix Figure~\ref{fig:eigen}.
% on downstream generation tasks.


% % \vspace{-0.5cm}
% \begin{figure}[ht]
%     \centering
%     % \adjustbox{trim={.1\width} {.1\height} {0.1\width} {.1\height},clip}
%     {\includegraphics[scale=0.5]{figs/eig_sbs.png} }
%     \vspace{-0.5cm}
%     \caption{\small Spectrum analysis of the self-attention matrix comparing the baseline (Dense) and our Sparse Prefix-Tuned (PT) transformer
% model zooming in on prefix parameters of size 100. The Y-axis is the normalized cumulative singular value of the self-attantion matrix \textbf{A}, and the X-axis the index of largest eigenvalue. The results are based on BART-Large on XSum dataset. The left plots the averages of all \textbf{A} on the lower layers, while right plots averages over higher layers.}%
%     \label{fig:eigen}%
%     \vspace{-0.3cm}
% \end{figure}
\noindent\textbf{Spectrum Analysis (Statistical Proof):} 
To investigate if our sparse models do in fact learn sparse representations, we conduct spectrum analysis on the encoder attention matrix \textbf{A} zooming in on the prefix parameters\footnote{A similar spectrum analysis has been used to prove the sparsity of the attention matrix in Linformer \citep{linformer}, a sparse transformer.}. To analyze the variation of attention scores we calculate the principal components of the attention scores of prefix parameters\footnote{Eigenvalues capture the variation of the
attention scores distribution along different principal components.}. We observe that the spectrum distribution of prefixes in lower layers is more skewed than in
higher layers, meaning that, in lower layers, more information is concentrated in the largest singular
values and the rank of \textbf{A} is lower. In summary, with sparse attention at the lower layers and dense attention at the top layers, the prefix-tuned models enables encoding salient features necessary for the factual and consistent summarization. Next, we empirically support this statistical proof.

\begin{table}[t!]
    \centering
    \small
    % \resizebox{1\textwidth}{!}{%
        \begin{tabular}{@{}l@{}c@{}c@{}c@{}c@{}c@{}}
        \hline 
        \textbf{Method} & \textbf{XSum} \ \ & \textbf{CNN} \ \ & \textbf{PubMed} \ \ & \textbf{Wikihow} \ \ & \textbf{SAMSum}\\
        \hline
        \multicolumn{6}{l}{\textit{\textbf{Finetune}}} \\
        \hline
        Dense   & 
        37.42 & 
        41.22 & 
        27.42 & 
        34.89 & 
        48.73 \\
        (\textit{a}) TruncSA  & 
        & 
        39.96& 
        & 
        & 
        48.12\\
        (\textit{b}) SoftSA  & 
        & 
        39.67& 
        & 
        32.53& 
        48.45\\
        \hline
        \multicolumn{6}{l}{\textit{\textbf{Prefix-tune}}} \\
        \hline
        Dense   & 
        35.47 & 
        39.08& 
        24.57& 
        28.27& 
        48.05\\
        (\textit{a}) TruncSA   & 
        35.39 & 
        39.52& 
        25.61& 
        28.94& 
        47.88\\
        (\textit{b}) SoftSA   & 
        & 
        39.24& 
        & 
        28.94& 
        \\
        (\textit{c}) HTruncSA \ \ \    &  
        36.42&  
        40.00&  
        25.28& 
        30.02& 
        48.00\\
        (\textit{d}) HSoftSA    &  
        36.13&  
        39.83& 
        24.90& 
        30.01& 
        48.33\\
    \hline
    \end{tabular}
    % }
    \vspace{-0.2cm}
    \caption{\small Sparse Attention experiment \textbf{ROUGE-L} results on Finetuning, and Prefix-tuning using dense and soft sparse attention designs in $\S$\ref{doessparseattentionlhelp}. 
    % Truncated (TruncSA) and Bernoulli Sampling soft attention (SoftSA) and Hierarchical Truncated (HTruncSA) and Soft Attention (HSoftSA) for Prefix-Tuning. 
    The best results accross models are \textbf{bolded}, second best results are also \underlined{\textbf{underlined}}. Full results are included in Appendix~\ref{apptab:sparse}.}
    \label{tab:sparse}
\end{table}

\noindent\textbf{Sparsity Analysis:} To further support the findings from the spectrum analysis, we investigate the impact of sparsity on the performance of the prefix-tuning models. For a fair comparison, we also apply attention sparsity on the finetuned models. We build prefix-tuning models with (\textit{a}) Truncated Sparse Attention (TruncSA), (\textit{b}) Soft Sparse Attention (SoftSA), (\textit{c}) Hierarchical TruncSA (HTruncSA), with top-\textit{p} sparsity at the lower layers, and dense attention at the top layers, (\textit{d}) Hierarchical Soft Sparse Attention (HSoftSA), with soft sparse attention at the lower layers but dense at top layers. 

We show the ROUGE-L results in Table~\ref{tab:sparse}. We observe that when sparsity is used on the prefix-parameters, the prefix-tuned models learn to encode more salient features about the summarization task and outperform baseline all-dense prefix-tuning models on all datasets. The performance improvements are more pronounced on long document summarization tasks such as Pubmed, reaching more than 2.0 ROUGE score improvements. %For datasets, such as extreme summarization, which requires learning of compositionality and abstraction to compose a single sentence short summary of a document, the hierarchical models still outperform prefix-tuned models. 
Comparing all layers sparse models of (\textit{a}) and (\textit{b}) to hierarchically biased sparsity models of (\textit{c}) and (\textit{d}), we observe improvements with the hierarchically structured sparse prefix-tuning models. More details on quantitative analysis are provided in Appendix~\ref{app:spectrum} and Table~\ref{apptab:sparse}.
% , suggesting that the prefix-parameters biased with a hierarchical structure yields better summaries.      


\begin{table}[t]
    \centering
    \footnotesize
    % \resizebox{1\textwidth}{!}{%
    \begin{tabular}{@{}lcc@{}}
        \hline 
        Dataset & \textbf{HierBlock} & \textbf{HierBlock+SoftSA} \\
        \hline
        Summarization & R1/R2/R-L & R1/R2/R-L \\
        \hline
        XSum &  43.91/20.83/36.38 &  \textbf{44.00}/\textbf{20.93}/\textbf{36.59}\\
        CNN/DM & \textbf{43.33}/20.27/\textbf{40.12} & \textbf{43.33}/\textbf{20.31}/40.10\\
        PubMED & \textbf{43.16}/\textbf{16.83}/24.87 & 42.96/16.64/\textbf{25.00}\\
        Wikihow & \textbf{39.34}/\textbf{15.55}/\textbf{28.75} &  39.30/15.42/28.67  \\
        SAMSum & 52.58/27.58/48.42 & \textbf{52.83}/\textbf{27.94}/\textbf{48.72}\\
        \hline
        \textbf{Struct-to-Text} & BLEU/R-L/CiDER & BLEU/R-L/BERT \\
        \hline
        E2E & 67.2/69.1/2.35 & \textbf{68.0}/\textbf{69.6}/\textbf{3.38}\\
        DART & & \\
        \hline
    \end{tabular}
    % }
    \vspace{-0.3cm}
    \caption{\small What happens when we introduce sparsity to hierarchically blocked prompt design? Summarization experiment results comparing dense and sparse prefix-tuning with structurally biased prefix design (via hierarchical blocking) on various text generation tasks. The best results across two models are \textbf{bolded}.}
    \label{tab:res3}
    \vspace{-0.3cm}
\end{table}

% ################################################
\subsection{Does sparsity on hierarchically blocked prefixes further improve performance?}
\label{sparsityinhierblock}
% ################################################
\noindent{\textbf{Finding:}} 
The most performance gains are obtained when
sparsity constraints are applied on the hierarchically blocked prefixes (Table~\ref{tab:res3}).

\noindent{\textbf{Analysis:}}
% Here we discuss ablations with respect to the sparsity methods applied on the hierarchically blocked prefix-models.
% The sparsity constraints imbued on the hierarchically structured prefix design improves the performance further on several summarization tasks, while the improvements are not statistically significant across all text generation datasets.  
% ################################################
Recall from the earlier discussions in $\S$\ref{blockingresults} that, if we apply blocking on the lower layered prefixes, while we let all tokens attend to all prefixes at the top layers (HierBlock models), we observe significant performance improvements. On separate set of ablations in $\S$\ref{doessparseattentionlhelp}, we also observe that if we introduce sparsity at different layers of the network, the sparse parameters influence the performance compared to the dense prefix tuned parameters at all layers. We now introduce sparsity on the hierarchically blocked prefix-models, combining the best hierarchically blocked prefix-tuned models with the sparse attention. 

In Table~\ref{tab:res3} we show results of our hierarchical prefix blocking (HierBlock) model against hierarchical prefix blocking model with soft sparse attention (HierBlock+SoftSA). To build the HierBlock+SoftSA models, we apply soft sparsity at the lower layers with blocked prefix parameters, while the top layers use dense prefixes with all tokens attending to all prefixes. In Table~\ref{tab:res3} we repeat the results of the last row from Table~\ref{tab:res1} for easy comparison.  We observe performance improvements on almost all the summarization tasks: XSum, CNN/DM, SAMSum, PubMED. We find that HierBlock+SoftSA models show significant improvements on SAMSum ($\pm$1.3; $p{<}$\num{1e-4}). On the structure to text generation tasks the sparsity on hierarchical blocking helps on some datasets (with E2E), though both HierBlock and HierBlock+SoftSA perform better than baseline prefix-tuning models (see App. Table~\ref{tab:res2}). More details are provided in Appendix~\ref{app:sparsityinhierblock}.

\begin{table}
\setlength{\tabcolsep}{3pt}
    \centering
    \small
        \begin{tabular}{rr|cccc}
        
        &  & \multicolumn{4}{c}{Wins \% matches} \\
        \multicolumn{2}{r|}{\textbf{Faithfullness}} & {PT} & {HSoftSA} & {HB+SoftSA} & {HB} \\
        \midrule
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Loses \%}}}
        & PT & & \win{\textbf{64.0}} & \win{{52.9}}& \win{\textbf{74.7}} \\[-0.25mm] 
        & HSoftSA & \lose{36.0} &  & \win{{46.4}} & \win{\textbf{65.3}}   \\[-0.25mm] 
        & HB+SoftSA & \lose{47.6} & \lose{53.6} & & \win{58.0} \\[-0.25mm] 
        & HB & \lose{25.3} & \lose{34.7} & \lose{42.0} & \\[-0.25mm] 
        \end{tabular}
% \vspace{.5cm}
        % \begin{tabular}{rr|cccc}
        % % \\
        % &  & \multicolumn{4}{c}{Wins \% matches} \\
        % \multicolumn{2}{r|}{\textbf{Coherence}} & {PT} & {HSoftSA} & {HB+SoftSA} & {HB} \\
        % \midrule
        % \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Loses \%}}}
        % & PT & & \win{\textbf{73.0}} & \win{{46.3}}& \win{\textbf{57.5}} \\[-0.25mm] 
        % & HSoftSA & \lose{27.0} &  & \win{{47.4}} & \win{{51.3}}   \\[-0.25mm] 
        % & HB+SoftSA & \lose{53.7} & \lose{52.6} & & \win{54.0} \\[-0.25mm] 
        % & HB & \lose{42.5} & \lose{48.7} & \lose{46.0} & \\[-0.25mm] 
        % \end{tabular}
        \begin{tabular}{rr|cccc}
        % \\
        &  & \multicolumn{4}{c}{Wins \% matches} \\
        \multicolumn{2}{r|}{\textbf{Overall}} & {PT} & {HSoftSA} & {HB+SoftSA} & {HB} \\
        \midrule
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Loses \%}}}
        & PT & & \win{\textbf{67.5}} & \win{{48.3}}& \win{\textbf{63.7}} \\[-0.25mm] 
        & HSoftSA & \lose{32.5} &  & \win{{47.3}} & \win{55.2}   \\[-0.25mm] 
        & HB+SoftSA & \lose{51.7} & \lose{52.7} & & \win{\textbf{57.3}} \\[-0.25mm] 
        & HB & \lose{36.3} & \lose{44.8} & \lose{42.7} & \\[-0.25mm] 
        \end{tabular}
    \vspace{-0.1cm}
    \caption{Human evaluation results on {\em Faithfullness} (top) and {\em Overall} (bottom) ratings. PT: Prefixtune, HSoftSA: Hierarchical Soft Attention, HB: HierBlock, HB+SoftSA: HierBlock with Soft Sparse Attention. Bold win \%s indicate significance ($p<.05$).}
    \label{tab:human_eval_pt}
\end{table}


% ################################################
\subsection{Do human evals. support our claims?}
\label{humanevals}
% ################################################
\noindent{\textbf{Finding:}} Humans generally prefer generated text from hierarchically blocked prefix-tuned models over all other models, find overall quality of generations indistinguishable from fine-tuning.

\noindent{\textbf{Analysis:}} To evaluate the generated text from our proposed methods against baseline models, we ask human annotators to rate generations on five criteria: \textit{faithfulness} (consistent with the context), \textit{relevance} (captures key-points), \textit{grammaticality}, \textit{coherence} (form a cohesive whole), and \textit{overall quality} (helpful, informative). Table~\ref{tab:human_eval_pt} shows the results of the study on faithfulness, and overall metrics. 
The columns show the percentage of wins of the model
against its opponent on a given row. Our Hierarhical Blocking (HierBlock) and  Hierarchical Soft Sparse Attention (HSoftSA) 
models beat prefix-tuning and HierBlock significantly ($p < .05$) beats most of our sparse models on all axes including factuality. In Table~\ref{apptab:humandetails} we provide comparisons with fine-tuning 
and observe that HierBlock models perform as good as finetuning on all criteria. More details about the evaluation setup as well as results on all the criteria comparing against fine-tuning and prefix-tuning can be found in Appendix~\ref{app:humanevals}.


% ################################################
\subsection{Which structural features are harder to transfer in low-resource settings?}
\label{lowdatasetting}
% ################################################
\noindent{\textbf{Finding:}} In low-resource settings, hierarchically designed sparse prefix parameters can efficiently transfer knowledge and represent the semantics and structure of input text yielding more accurate output generations. 
% When they are further enriched with the sparse features, they outperform finetune and prefix-tune baselines.    

\noindent{\textbf{Analysis:}} We simulate a low-resource setting by randomly sampling \textit{k}\% (k={5,10,25,50}) from the training dataset of two summarization tasks: XSum on news, and Wikihow on DIY domains (see train data sizes in Table~\ref{tab:datasets}). 
We use the same hyperparameter settings as our previous models detailed in $\S$~\ref{setup}. We compare our approach to finetuning and prefix-tuning under low-resource settings.
% For reference we also provide the result of our baseline fine-tuning and prefix-tuning systems on the full training data.    

% % ########################################
% \subsection{Human Evaluations} 
% \label{human}
% % ########################################
% \paragraph{Finding:}
% \paragraph{Analysis:} 

\begin{wrapfigure}{r}{0.2\textwidth}
  \vspace{-12pt}
     \begin{tikzpicture}[yscale=0.40, xscale=0.40] 
     \begin{axis}[
     font=\fontsize{15}{0}\selectfont,
     xmax=50,xmin=0,
     ymin= 27.5,ymax=31.5,
     xlabel=\emph{\% train samples}
    %  ,ylabel=\emph{Rouge-L},
     xtick={5,10,25,50},
     ytick={27,28,29,30,31},
     legend columns=2, 
    %  legend style={legend pos=north west}
     legend style={at={(0.5,1.15)},anchor=north},line width=1pt,
     ]
     \addplot [green!60!black,mark=square] coordinates{ (5,28.45) (10,29.09) (25,30.53) (50,31.05)};
     \addplot [olive,mark=x] coordinates{ (5,27.87) (10,28.79) (25,29.78) (50,30.27)};
     \addplot [blue,mark=*] coordinates{ (5,28.54) (10,29.21) (25,30.09) (50,30.68)};
     \addplot [red,mark=o] coordinates{ (5,28.94) (10,29.71) (25,30.38) (50,30.60)};
          \legend{\emph{Finetune},\emph{Prefix-tune},\emph{HierBlock},\emph{HierBlock+SA}}
     \end{axis} 
     \end{tikzpicture}
\caption{\small Average ROUGE-L scores on \textbf{low-resource settings}.} 
% Our structurally biased parameter tuned HierBlock (\textcolor{blue}{blue}) and HierBlock+SA (\textcolor{red}{red}) consistently outperforms the baseline Finetuned (\textcolor{green!60!black}{green}) and Prefix-tuned models (\textcolor{olive}{olive}) when <50\% training data is used.}
\label{fig:low_small}
  \vspace{-10pt}
\end{wrapfigure}


In Figure~\ref{fig:low_small} on the right, we plot ROUGE-L averaging scores of models trained on XSUM and Wikihow. Our structured prefix-tuned models, HierBlock (\textcolor{blue}{blue}) and its sparse extension which uses sparse features, HierBlock+SA (\textcolor{red}{red})
outperforms fine-tuned (\textcolor{green}{green}) and prefix-tuned models (\textcolor{olive}{olive}), while using the same number of parameters in low resources settings (when <50\% training samples are used). 
Although HierBlock models show consistent performance, on low-resource settings HierBlock-SA performance is more stable.
(See Appendix~\ref{app:lowdatasetting} for more details.)


==> old/model.tex <==
% ################################
\section{Discourse Aware Prompt Design}
\label{discourse}
% ################################
\noindent\textbf{Visualizing prompt impact.} 
% We start with our intuition for discourse-aware prompt design approaches for efficient prefix-tuning. 
To motivate the discourse-aware prompt design, we investigate the impact of prefix-parameters on transformer models during prefix-tuning. 
We first analyze the attention behaviour similar to \citep{sun-lu-2020-understanding}. We prefix-tune two \textsc{Bart-Large} models, one on structure-to-text generation task with E2E dataset \citep{e2e}, and another on summarization with CNN/DM \citep{hermann2015teaching}. For E2E we use 10-prefixes (the first 10 keys are from prefix parameters) and 100-prefixes for CNN/DM\footnote{The length of per instance input tokens is 680 in CNN/DM and 26 in E2E dataset, so we use less prefix parameters. \textcolor{red}{add percent improvement of parameters}}. In Figure~\ref{fig:attn}, we plot the encoder self-attention distributions \textbf{\textit{A}} for different layers averaging over all head vectors. The \textit{x}-axis represent the keys while y-axis denote the queries. For attention matrices of all the layers, see Appendix \ref{app:prefixvisual} Figure~\ref{app:fig:attn}. The attention scores show stronger relations with the prefix-keys in the E2E model compared to CNN/DM, where the prefixes exhibit weaker relations compared to the 
input keys. We attribute this to a few issues which we investigate in this work: 

\noindent\textbf{Modeling hierarchical structure.} Firstly, during prefix-tuning, the model should not only focus on learning the task specific semantics, but also the models should learn the corresponding discourse structure of the downstream task datasets. To model the intrinsic structure of input text, biasing transformer models with a type of hierarchy has been shown to improve the generation performance. For example, previous work \citep{cohan-etal-2018-discourse,liu2019} learns the discourse structure of human written text (e.g., the beginning, body, conclusion paragraphs, topic shifts, etc.) with hierarchically structured transformers to capture the salient aspects in the input text necessary for improved performance in summarization.
% Similarly, imbuing the transformers at different layers of the network with a type of structural bias that represents the syntactic structure and semantic content \citep{jiang-etal-2021-enriching} improves summarization performance. 
With probing experiments \citet{jawahar-etal-2019-bert} show that BERT \cite{bert}
captures surface features and phrase-level information in the lower layers, 
syntactic features in the middle and semantic features and long-distance dependencies at the higher layers. Motivated by these, we introduce variations of \textbf{hierarchical blocking} on prefix parameters at different layers of the network and investigate their impact on text generation with qualitative and quantitative experiments. 


\noindent\textbf{Introducing sparsity.} Secondly, the weaker prefix attention in longer inputs (Figure~\ref{fig:attn}-CNN/DM attention matrices) may imply that the attention neglects important connections, and potentially disturbed by many unrelated words. 
This issue can be attributed to the softmax function at attention score calculation \citep{Laha2018OnCS,cui-etal-2019-fine}. Softmax produces attention distribution with dense dependencies between words, and fails to assign near/exactly zero probability to less meaningful relations.
Thus, the model neglects to pay more attention to important connections while also being easily disturbed by many unrelated words \citep{cui-etal-2019-fine}. This issue is more pronounced in tasks like abstractive summarization, since only a handful of salient input aspects is needed to compose a coherent summary. Sparse attention mechanisms \cite{liu2021hetformer,Shi2021SparseBERTRT} can remedy this issue by learning to avoid attending to the content unrelated to the query. We introduce soft-attention blocking on the prefix and input parameters to put emphasis on important prefixes and tokens. 


Below we describe ways to apply a suite of blocking schemes and sparsity in prefix-tuning models as sketched in Figure~\ref{fig:sparseattn}. Each block represents attention matrix  $\mathbf{A}$$\in$$\textstyle \mathbb{R}^{T \times (P+T)}$, of 
each token $a_t$$\in \mathbb{R}^{(P+T)}$ (row vector) denoting to attention weights of all $P$ prefix and $T$ input-key features.
% that are to be applied on their corresponding value vectors $v_{n}$, $n$=1$\cdots (P+T)$. 

% In prefix-tuning, the $\mathbf{A}$$\in$$\mathbb{R}^{T \times (P+T)}$ matrix columns correspond to $P$  prefix-key and $T$ input-key features. 
% $n$=\{1$\dots (P+T)$\}

% ################################
\subsection{Prefix Blocking}
\label{prefixblocking}
% ################################
As shown in Figure~\ref{fig:sparseattn}-(b) and (e), the
two variations of prefix-blocking we introduce here are a type of structural bias we imbue the models to simulate high-level discourse structure of documents: 
% (e.g., paragraphs, topics, etc.):

\noindent\textbf{(\emph{i}) Uniform Blocking (UniBlock)}: 
 We first split the sequence of input tokens into segments. We allocate different sets of prefix parameters to each segment and apply blocking on the rest of the prefix parameters.   
% Specifically, in the self-attention setting, the input tokens of a segment only prepends a set of key and value prefixes designated to that segment, while each token can attend to all tokens. 
In baseline prefix-tuning, a query of a token can bind with all the prefix and input key and value parameters, while in the uniform blocked prefix-tuning, the query of a token in the input or output segment can bind with all input key and values but only with the designated prefix key and value vectors. 
For example, if 100 prefix parameters are used and we split the input tokens into 2 segments, the first 50 prefix keys and values can only be bound with the query vectors of input tokens from the first input segment and so on. 
We only apply blocking to the prefix parameters and let all inputs tokens  attend to each other, see Figure~\ref{fig:sparseattn}-(b).   
In uniform blocking, we use the same blocking schema at each layer. 

\noindent\textbf{(\emph{ii}) Hierarchical Blocking (HierBlock)}: 
To bias the prefix parameters with a form of hierarchy, we use the uniform prefix-blocking on the lower layers of the transformer, while we let all tokens attend to all prefixes at the top layers  as shown in Figure~\ref{fig:sparseattn}-(e).
The attention matrix of the top layers is same as the standard prefix-tuning of \citep{prefixtune} where no blocking on prefixes is applied.
\begin{figure}[t]
    \centering
    \adjustbox{trim={0\width} {.02\height} {0\width} {0\height},clip}
    {\includegraphics[width=0.48\textwidth]{figs/blocks_small.png} }
    \vspace{-0.5cm}
    \caption{\small Skectches if attention matrices \textbf{\textit{A}} used in prefix-tuning models representing different prefix design patterns.
    % for input sequence of two tokens ($T$=2) with two additional prefixes ($P$=2). 
    $p$-keys and $i$-keys denote $P$ prefix and $T$ input keys. 
    % (a) baseline prefix-tuning dense attention, each query row bind with the column prefix- and input-keys, (b) uniform blocking applies prefix-blocking to all layers, (c) hierarchical-blocking applies prefix blocking on lower layers while keeping dense prefixes at higher layers, (d) truncated attention uses top-\textit{p} sampling to block some of prefix or input parameters, while (e) uses soft sampling to sparsify the prefix and input attention scores, (f) introduces sparsity to the hierarchical blocking with soft sparse attention. Green and yellow cells represent prefix and input keys respectively. 
    Sparsity of attention scores are indicated by color gradations. White cells in any row represent blocked input & prefix parameters for the query.}%
     \vspace{-0.3cm}
    \label{fig:sparseattn}%
\end{figure}

% ################################
\subsection{Sparse Attention Prefix-Tuning}
\label{sparseattnpt}
% ################################
To train a prefix-tuning model that learns to highlight important input content, we introduce four sparse attention design options for the encoder. 

% ################################
\noindent\textbf{(\emph{a}) Truncated Sparse Attention (TruncSA)}:
% ################################
\citet{dai-etal-2021-multimodal} used
 sparse cross-attention using truncation to improve salient feature extraction which showed improvements in downstream tasks performance. Following this intuition, to simulate encoding with salient features, we apply top-\textit{p} truncation on both the prefix and input keys as follows: we first add all the row elements $a_{ti}$ $\in $[0,1] of the attention matrix, namely the attention scores contributing from all the queries, then normalize across all key-features, which yields a key-feature impact row vector $\Tilde{a}_t$ $\in \mathbb{R}^{(P+T)}$ and $\Tilde{a}_i \in \mathbf{\Tilde{a}}$:
\begin{equation}
\vspace{-0.2cm}
    \bar{a}_n = \textstyle \sum_i^{T} a_{ti} \quad \Tilde{a}_t = \bar{a}_t/(\sum_n^{(P+T)} \bar{a}_n)
\end{equation}
Using top-\textit{p} truncation \citep{dai-etal-2021-multimodal} we truncate the feature key scores and use 
the top-\textit{p} portion of the probably mass in each key attention score.  
We create a binary mask for each key feature via $mask(\mathbf{\Tilde{a}}) = \text{top-}p(\mathbf{\Tilde{a}}, \tau)$ by assigning 1.0 to the keys that the top-\textit{p} sampling has selected, 0 otherwise and threshold parameter $\tau$ controls sparsity.
% \begin{equation}
%     mask(\mathbf{\Tilde{a}}) = \text{top-}p(\mathbf{\Tilde{a}}, \tau) 
% \end{equation}
% We control the degree of sparsity of the attention with threshold parameter $\tau$.
Lastly, we broadcast point-wise multiplication between the sparse mask and the attention matrix  $\mathbf{A}$ to obtain the top-\textit{p} sparse attention matrix $\Tilde{\mathbf{A}} = mask(\mathbf{\Tilde{a}}) \odot \mathbf{A}$, as sketched in Figure~\ref{fig:sparseattn}-(c). 

% \begin{equation}
%     \Tilde{\mathbf{A}} = mask(\mathbf{\Tilde{a}}) \odot \mathbf{A}
% \end{equation}
Our top-\textit{p} truncation is similar to using dropout on the features of the network during training while controlling the dropout rate with a user-defined threshold to compensate for overfitting and performance. 
% We use dense attention at inference time. 
Although top-\textit{p} sparse attention provides automatic control over attention sparsity, truncation completely masks some features. 
Next, we show how to dynamically learn to apply \textit{soft}-sparsity via sampling from a distribution. 

% ################################
\par \noindent\textbf{(\emph{b}) \textit{Soft} Sparse Attention (SoftSA)}:
% ################################
% In \cite{Shi2021SparseBERTRT}, the authors investigate the degree of self-attention sparsity and suggest that a token can attend to more tokens with low sparsity given the same amount of computational cost, and is thus expected to have better performance. On the other hand, at high self-attention sparsity, model performance may drop. 
% An alternative to attending to heuristically (i.e., top-\textit{p}) or randomly selected tokens, is 
Influencing the attention distribution with a stochastic mask to attend to salient tokens can potentially help build higher quality sparse attention for text modeling.
Several work investigate novel approaches to learn the sparsity in attention matrix \cite{Li2021EASEES,10.1162/tacl_a_00353,Shi2021SparseBERTRT} using a sampling method to formulate the right amount of sparsity. They associate the attention scores $a_{t,i}$ with each position ($t,i$) in $\mathbf{A}$ and define a sampling distribution to learn the attention mask during training as sketched in Figure~\ref{fig:sparseattn}-(d). Similarly, we define relaxed Bernoulli distribution as a sampler to construct our stochastic mask. 
Since sampling from Bernoulli distribution is not differentible, we use the
Gumbel Softmax reparameterization trick \citep{jang2017categorical}
with gumbel-softmax:
\vspace{-0.3cm}
\begin{equation}
\tilde{a}_{tn} = \underset{n \in 1\dots (P+T)}{\text{Softmax}} \left(a_{t,n},g,\tau\right)
\end{equation}
\noindent where $g$=$-\log(-\log(u))$ is an independent Gumbel noise generated
from the uniform distribution $u \sim U(0, 1)$
% \begin{equation}
% g = -\log(-\log(u)), u \sim U(0, 1),
% \end{equation}
and $\tau$ is a temperature. 
As $\tau$ approaches zero, the gumbel output approaches to a discrete distribution in \{0, 1\}, becomes identical to
those from the Bernoulli distribution. For details on Gumbel-softmax reparameterization trick, see Appendix~\ref{app:hyperparameters}.
% We use $\tau\in$[1.0, 0.1, 0.01]. 

% ################################
\noindent\textbf{(\emph{c \& d}) Hierarchical Sparse Attention}:
% ################################
To simulate an intrinsic discourse structure of the input text, similar to the hierarchical blocking in $\S$~\ref{prefixblocking}, we apply sparsity on the parameters only at the lower layers. We train hierarchical models with the dense attention at the higher layers, and apply (\textit{c}) \textit{truncated} (\textbf{HTruncSA})  or (\textit{d}) \textit{soft} sparse attention (\textbf{HSoftSA}) at the lower layers (see Figure~\ref{fig:sparseattn}-(f)).
% We also train with the opposite masking schema where we use sparse attention at the higher layers and dense at the lower layers which constantly performed worse.
% ################################
\par \noindent\textbf{(\emph{e}) Hierarchical Blocking with Sparse Attention (HierBlock+SoftSA)}:
% ################################
The hierarchical blocking models we introduced in $\S$~\ref{prefixblocking} puts restrictions on the prefix parameters that input tokens can bind with at different layers of the network. To analyze the impact of ensemble of prefix blocking and sparsity, we introduce sparsity to the hierarchically blocked prefix-tuning models. 
We apply soft sparsity (SoftSA) on the lower layers of the network attention matrices of HierBlock models and keep the higher layer attention matrices dense. 

==> old/related_long.tex <==
% ################################
\section{Related Work}
% ################################
\textbf{Prompt Based LM Tuning.} 
Recent years have observed several efficient methods for tuning large-scale pre-trained language models, which are generally referred to as prompt-tuning. \citet{prompttuning_survey}  provide an extensive discussion of the recent methods varying from prompt engineering \citep{petroni-etal-2019-language,cui-etal-2021-template}, which learns important inputs for prompting methods, answer engineering \citep{jiang-etal-2020-know,jiang-etal-2020-x}, which designs models to search for an answer space and then maps to the output space, to more advanced approaches such as prompt ensembling \citep{Mao2021UniPELTAU}, prompt composition \citep{hanpromptcomp}, prompt augmentation \citep{gao-etal-2021-making}, and prompt-aware training methods \citep{Lester2021ThePO,prefixtune}. \citet{prefixtune} propose “prefix tuning” and show strong results on some text generation tasks, leaving room for generalization to all generation tasks. Here, we build directly upon
the prefix-tuning from \citet{prefixtune}, showing
where it falls short and providing several discourse-aware prompt design approaches. 
In particular, we find that the
method struggles with encoding the salient concepts that most 
text generation models require. This setting bears similarities to 
discourse modeling, which we discuss below.

\noindent\textbf{Discourse Modeling.} The early work on discourse analysis for text generation tasks \citep{marcu-1997-discourse}, have shown that the concepts of rhetorical analysis can be used effectively to detect the most important units in text.
A larger family
of methods make architectural design choices 
to teach models about the overall document discourse structure
\citep{coherence, coherence2, coherence3,Barzilay2004CatchingTD} and improve document summarization.
Recent work implement different modeling choices or architectures to model the discourse structure via: structured attention modeling \citep{cohan-etal-2018-discourse}, graph based methods \citep{dong-etal-2021-discourse}, hierarchical encoders \citep{pasunuru2021data}, to name a few. We simulate the discourse structure by incorporating some of the findings from earlier work such as hierarchical encoders and propose discourse-aware prompt-design for frozen language models.

\noindent\textbf{Sparse Language Models.} 
Most work on sparsity in transformers aim at improving the time and space 
bottleneck of the dense transformers \citep{tay2021long}. 
Works on coherent text generation introduce different sparsity methods 
for text generation tasks to
favor performance in terms of coherence, fluency and consistency,
fewer repetitions, and n-gram diversity closer
to human text. These work range from: sparse methods on 
posterior vocabulary distributions at inference time \citep{Fan2018HierarchicalNS,nucleus}, sparse encoders \citep{cui-etal-2019-fine}, sparse attention mechanisms \cite{liu2021hetformer,Shi2021SparseBERTRT, expirespan}, 
modified softmax \citet{Martins2020SparseTG}, or loss functions with additional terms \citep{unlikelihood} at training time to improve LM coherence. Following these work, our proposed approaches introduce sparsity on the attention matrix focusing on improving the knowledge transferred to the downstream tasks.




% Recently,
% thanks to the success of GPT-3 (Brown et al., 2020),
% various prompting strategies including discrete natural language prompt (Shin et al., 2020; Gao et al.,
% 2020), continuous prompts (Liu et al., 2021b; Li
% https://github.com/thunlp/PromptPapers
